VeriSolid: Correct-by-Design Smart Contracts for Ethereum

The adoption of blockchain based distributed ledgers is growing fast due to their ability to provide reliability, integrity, and auditability without trusted entities. One of the key capabilities of these emerging platforms is the ability to create self-enforcing smart contracts. However, the development of smart contracts has proven to be error-prone in practice, and as a result, contracts deployed on public platforms are often riddled with security vulnerabilities. This issue is exacerbated by the design of these platforms, which forbids updating contract code and rolling back malicious transactions. In light of this, it is crucial to ensure that a smart contract is secure before deploying it and trusting it with significant amounts of cryptocurrency. To this end, we introduce the VeriSolid framework for the formal verification of contracts that are specified using a transition-system based model with rigorous operational semantics. Our model-based approach allows developers to reason about and verify contract behavior at a high level of abstraction. VeriSolid allows the generation of Solidity code from the verified models, which enables the correct-by-design development of smart contracts.

==> CfromSolidity.tex <==
\section{Translating Solidity to C}
\label{sec:Ctranslation}

\subsection{Basic Types}
Assuming a 64-bit architecture for C:
\begin{center}
\begin{tabular}{|l|l|}
\hline
Solidity & C \\ 
\hline
\texttt{uint64 x;} & \texttt{unsigned int x;} \\
\texttt{int64 x;} & \texttt{int x;} \\
\texttt{bool x;} & \texttt{int x;} \\
\texttt{bytes32 x;} & \texttt{char x[32];} \\
\texttt{address x;} & \texttt{char x[20];} \\
\hline
\end{tabular}
\end{center}
Note that \texttt{bytes32} and \texttt{address} work as value types in Solidity, not as references. So operators (e.g., arithmetics and comparisons) work on the values, in contrast with C, where the operators would work on the references. This means that \texttt{x == y} in Solidity (assuming that \texttt{x} and \texttt{y} are of type \texttt{bytes32} or \texttt{address}) is equivalent to \texttt{memcmp(x, y, sizeof(x)) == 0} in C.

\subsection{Type Definitions}

\subsubsection{Enum}\ \\
Solidity:
\begin{verbatim}
enum TypeName { A, B, ... };
\end{verbatim}
C:
\begin{verbatim}
typedef enum { A, B, ... } TypeName;
\end{verbatim}

\subsubsection{Struct}\ \\
Solidity:
\begin{verbatim}
struct TypeName {
  Type1 Member1;
  Type2 Member2;
  ...
}
\end{verbatim}
C:
\begin{verbatim}
typedef struct {
  Type1 Member1;
  Type2 Member2;
  ...
} TypeName;
\end{verbatim}

\subsection{Mapping}
Solidity:
\begin{verbatim}
mapping(Type1 => Type2) Var;

Var[x] = y;

y = Var[x];
\end{verbatim}
C:
\begin{verbatim}
Type1 *VarFrom = null;
Type2 *VarTo = null;
int VarSize = 0;
void VarPut(Type1 x, Type2 y) {
  if (VarSize == 0) { // first element
    VarFrom = malloc(sizeof(Type1));
    VarFrom[0] = x;
    VarTo = malloc(sizeof(Type2));  
    VarTo[0] = y;
    VarSize = 1;
  }
  else {
    for (int i = 0; i < VarSize; i++) 
      if (VarFrom[i] == x) { // value comparison!
        VarTo[i] = y; // existing element
        return;
      }
    // new element
    VarFrom = realloc(VarFrom, sizeof(Type1)*(VarSize + 1));
    VarFrom[VarSize] = x;
    VarTo = realloc(VarTo, sizeof(Type2)*(VarSize + 1));
    VarTo[VarSize] = y;
    VarSize++;
  }
}
void VarGet(Type1 x, Type2 y) {
  for (int i = 0; i < VarSize; i++)
    if (VarFrom[i] == x) // value comparison!
      return VarTo[i];
  return 0; // value return!
}

VarPut(x, y);

y = VarGet(x);

\end{verbatim}

\begin{comment}
\subsection{Blind Auction in C}

\begin{lstlisting}[style=customjava]
typedef enum {
  States_ABB,
  States_RB,
  States_F,
  States_C
} States;

States state = States_ABB;

typedef struct {
  char blindedBid[32];
  unsigned int deposit;
} Bid;

typedef struct {
  Bid *bids;
  int length;
} BidArray;

void BidArrayPush(BidArray *bidArray, Bid bid) {
  if (bidArray->length == 0) {
    bidArray->bids = (Bid*) malloc(sizeof(Bid));
    bidArray->bids[0] = bid;
    bidArray->length = 1;
  }
  else {
    bidArray->bids = (Bid*) realloc(bidArray->bids,
                (bidArray->length + 1) * sizeof(Bid));
    bidArray->bids[bidArray->length] = bid;
    bidArray->length++;
  }
}

mapping(char[20] => BidArray) bids;
mapping(char[20] => uint) pendingReturns;

char highestBidder[20];
unsigned int highestBid;
time_t creationTiem = time(); 
    
void bid(char blindedBid[32]) {
  // Guards
  if (state == States_ABB) {
    // Actions
    // create struct
    Bid _bid;
    _bid.blindedBid = blindedBid;
    _bid.deposit = msg.value;
    // store struct
    BidArray bidArray = bidsGet(msg.sender);
    BidArrayPush(*bidArray, _bid);
    bidsPut(msg.sender, bidArray);
    pendingReturnsPut(msg.sender,
      pendingReturnsGet(msg.sender) + msg.value));
  }
}
    
void close() {
  // Guards
  if (state == States_ABB &&
        time() >= creationTime + 5 * 24 * 60 * 60) {
    state = States_RB;
  }
}

void reveal(unsigned int values[], int values_length, 
            char secrets[], int secrets_length) {
  if (state == States_RB &&
        values_length == secrets_length) {
    BidArray bidArray = bidsGet(msg.sender);
    for (int i = 0; 
         i < (bidArray.length < values_length ? 
           bidArray.length : values_length); 
         i++) {
      Bid bid = bidArray.bids[i];
      unsigned int value = values[i];
      char *secret = &secrets[i * 32];
      char hash[32];
      keccak256(hash, value, secret);
      if (memcmp(bid.blindedBid, hash, 32) != 0)
        continue;
      if (bid.deposit >= value && 
            value > highestBid) {
        highestBid = value;
        highestBidder = msg.sender;
      }
    }  
  }
}
    
void finish() {
  // Guards
  if (state == States_RB &&
        time() >= creationTime + 10 * 24 * 60 * 60) {
    // Actions
    state = States_F;
  }
}
    
void cancelABB() {
  // Guards
  if (state == States_ABB) {
    // Actions
    state = States_C;
  }
}
    
void cancelRB() {
  // Guards
  if (state == States_RB) {
    // Actions
    state = States_C;
  }
}

void withdraw() {
  // Guards
  if (state == States_F) {
    // Actions
    unsigned int amount = 
          pendingReturnsGet(msg.sender);
    if (amount > 0 &&
          memcmp(msg.sender, highestBidder) != 0) {
      msg.sender.transfer(amount);
      pendingReturnsPut(msg.sender, 0);
    }
    else {
      msg.sender.transfer(amount - highestBid);       pendingReturnsPut(msg.sender, 0);
    }
  }
}
    
void unbid() {
  // Guards
  if (state == States_C) {
    // Actions
    unsigned int amount = pendingReturnsGet(msg.sender);
    if (amount > 0) {
      msg.sender.transfer(amount);
      pendingReturnsPut(msg.sender, 0);
    }
  }
}

\end{lstlisting}
\end{comment}



==> parityWallet.tex <==
\section{Parity Wallet Model Explained}
\label{sec:wallet}

We created the transition systems (shown in Figure~\ref{fig:wallet}) modeling the behavior of the library and a wallet contract. To make the models of \texttt{WalletLibrary} and \texttt{Wallet}, we use the \texttt{*\_library} and \texttt{*\_wallet} notation, respectively, for representing the following set of functions.
\begin{itemize}
\item \texttt{$*\_$library} represents the {\ttfamily execute, addOwner,} {\ttfamily changeRequirement, setDayLimit, removeOwner, confirm, resetSpentToday, changeOwner, revoke, hasConfirmed, isOwner} functions;
\item \texttt{$*\_$wallet} represents the  fallback, {\ttfamily hasConfirmed, isOwner} functions.
\end{itemize}

The functions of the library, i.e., {\ttfamily $*\_$library, initWallet,} {\ttfamily initDayLimit, initMultiOwned, kill} can be called directly in the \texttt{WalletLibrary} and executed with the corresponding transitions. Additionally, any \texttt{Wallet} can delegate the call to any of these functions through the binary BIP connectors. The \texttt{delegate} transition represents any call delegation to the {\ttfamily $*\_$library, initWallet, initDayLimit, initMultiOwned, kill} functions of the \texttt{WalletLibrary}. In particular, \texttt{initial} delegates to \texttt{initDayLimit} and \texttt{initMultiOwned}, \texttt{*\_wallet} delegates to some function in \texttt{*\_library}, and \texttt{kill} delegates to \texttt{kill}. 

The states of the \texttt{WalletLibrary} and \texttt{Wallet} contracts can be explained as follows:
\begin{itemize}
\item \texttt{Start}: initial state of the contract after creation. Note that the contract does not have a constructor, so all variables are zero.
\item \texttt{Initialized}: main state of the contract, which is entered when the owners are set up.
\item \texttt{Destroyed}: final state of the contract, which is entered when the contract is killed by an owner. Note that the contract is completely dysfunctional in this state (no functions may be called), and its stored value has been transferred to another address.
\end{itemize}

